A Theory of Usable Information Under Computational Constraints

We propose a new framework for reasoning about information in complex systems. Our foundation is based on a variational extension of Shannon's information theory that takes into account the modeling power and computational constraints of the observer. The resulting \emph{predictive $\mathcal{V}$-information} encompasses mutual information and other notions of informativeness such as the coefficient of determination. Unlike Shannon's mutual information and in violation of the data processing inequality, $\mathcal{V}$-information can be created through computation. This is consistent with deep neural networks extracting hierarchies of progressively more informative features in representation learning. Additionally, we show that by incorporating computational constraints, $\mathcal{V}$-information can be reliably estimated from data even in high dimensions with PAC-style guarantees. Empirically, we demonstrate predictive $\mathcal{V}$-information is more effective than mutual information for structure learning and fair representation learning.

==> old_definition.tex <==
Before we formally define the predictive $\F$-information, we first define the $\F$-Entropy as a measure of the uncertainty in a random variable.
% \js{i feel like the $\n$ symbol is ugly, maybe use the $\varnothing$ symbol instead?}\s{agreed, maybe let's macro it?}

\textbf{Regularity Conditions:} To minimize technical overhead we restrict out discussion only to distributions with probability density functions (PDF) or probability mass functions (PMF) with respect to the underlying measure. %We also assume that the underlying measure is either the counting measure (discrete) or the Lesbegue measure in multi-dimensional real space (continuous). 

\begin{definition}[Predictive $\F$-entropy]
Let $Y$ be a random variable taking values in $\mathcal{Y}$. \s{do we want this to be discrete?} \js{not necessarily? if Y is continuous then we are just not considering some non-discrete measure, which should be implied from $\gP(\gY)$?}\yx{the $\gP(\gY)$ can be both continuous and discrete. Do we need to define them separately. I think there are only some minor difference of properties between continuous and discrete Y}\sj{We need to assume some additional regularity conditions, for example the distribution could be neither discrete nor continuous}
Let $\mathcal{P}(\mathcal{Y})$ be the set of all probability density functions over $\mathcal{Y}$. Let $\Omega^{\n}=\{f:\{\n\} \rightarrow \mathcal{P}(\mathcal{Y})\}$, and $\mathcal{F} \subseteq \Omega^\n$. Then the predictive $\F$-entropy is defined as
\begin{equation}
H_{\F}(Y) = \inf_{f \in \F} \mathbb{E}_{y \sim Y}\left[\log \left( \frac{1}{f[\n](y)}\right)\right]
\end{equation}
\end{definition}

% \s{worth explaining the $f[\n](y)$ notation }
% \s{fix typesetting of $($ before a fraction using left and right}
% https://math.stackexchange.com/questions/273330/why-is-a-nullary-operation-a-special-element-usually-0-or-1
 Note that $f[\n]$ is the density function %with $\n$ as its inverse image, 
 and $f[\n](y) \in \mathbb{R}$ is the density function's value at $y$. $H_{\F}(Y)$ can be interpreted  %as the smallest expected negative log likelihood of the predicted variable, over all distributions in the range of $\F$. It can also be recognized 
 as the smallest cross entropy between the true underlying distribution of $Y$ and the distributions in the set $\{f[\n]\mid f\in \F\}$. 
 
 The complexity of $\F$ purely lies on the diversity of density functions in the set $\{f[\n]\mid f\in \F\}$, since the domain of all the functions in $\F$ is a singleton. However, when taking the concept of "predictive" of another random variable $X$ to $Y$ into account, the complexity of the mapping from $X$ to the density function of $Y$ emerges. Based on such intuition, we define the conditional $\F$ entropy as follows: 
%Based on the definition of the 
\begin{definition}[Predictive conditional $\F$-entropy]
Let $X,Y$ be two random variables taking values in $\mathcal{X} \times \mathcal{Y}$. Let $\mathcal{P}(\mathcal{Y})$ be the set of all probability density functions over $\mathcal{Y}$. Let $\Omega=\{f:\mathcal{X} \rightarrow \mathcal{P}(\mathcal{Y})\}$, and $\mathcal{F} \subseteq \Omega$. Then the predictive conditional $\F$-entropy is defined as
\begin{equation}
\label{eq:cond_entropy}
H_{\F}(Y | X) = \inf_{f \in \F} \mathbb{E}_{x,y \sim X,Y}\left[\log\left(\frac{1}{f[x](y)}\right)\right]
\end{equation}
\end{definition}
% \s{i think we should change $x \sim X, y \sim Y$ to $x,y \sim X,Y$, to suggest joint sampling}
% Written in this form,  $H_{\F}(Y| X)$ not only incorporate the expressive power of the distributions, but also the complexity of the mapping $\mathcal{X} \mapsto \mathcal{P}(\mathcal{Y})$. 

% \s{explain the intuition before moving one. explain in words (and refer to later proposition) how using omega one gets standard entropy. give some intuition for what this F is }

Similar to the predictive entropy, the predictive conditional entropy chooses the observer's capacity by choosing $\F \subset \Omega$. % as the variational family. 
As shown in proposition \ref{prop:property}, if the $\F$ is the largest possible, i.e. $\F = \Omega$, then the 
infimum in Eq.(\ref{eq:cond_entropy}) is achieved by
%best approximation function in $\F$ is 
the true conditional density function, and we have $H_{\F}(X|Y) = H(X|Y)$. After we define $H_{\F}(Y|X)$ and $H_{\F'}(Y)$ for some choice of $\F$ and $\F'$, we can define a notion of ``mutual information'', which is the reduction of entropy after conditioning on $X$. However, for this mutual information to possess several desirable properties, we need an extra condition on $\F$ and $\F'$. 
\s{how about we remove optional ignorance as a requirement in the F-MI definition? instead, say that MI will be non-negative if it satisfies that property. i feel it is confusing and a bit messy. seems more of a technicality that we should try to ``hide''}\yx{I recommend we still keep the optional ignorance requirement, since it guarantees the non-negativity of F-information. What's more, we require this property in some proofs.}
%For several reasonable properties of mutual information to hold, we need an additional requirement. 
\begin{definition}[Optional-ignorance]
Let $\mathcal{P}(\mathcal{Y})$ be the set of all probability distributions over $\mathcal{Y}$. A set of functions $\F \subset \lbrace f: \mathcal{X} \rightarrow P(\mathcal{Y}) \rbrace$ is optional-ignorance w.r.t a set of functions $\F' \subset \lbrace f: \{\n\} \rightarrow P(\mathcal{Y}) \rbrace$ if the following property hold:

\begin{equation}
\forall f' \in \F', \exists f \in \F \text{ s.t. } \forall x \in \mathcal{X}, f(x) = f'[\n]
\end{equation}
\end{definition}
Optional ignorance is easy to satisfy. For example, for any set of distributions $\lbrace p_\theta(y) \vert \theta \in \mathbb{R}^d \rbrace$ indexed by $d$ real parameters $\theta \in \mathbb{R}^d$, if we choose $\F' = \lbrace \lbrace \n \rbrace \to p_\theta \vert \theta \in \mathbb{R}^d \rbrace$, and $\F$ is defined by a neural network mapping $x \in \mathcal{X}$ to $\theta$, then optional ignorance is automatically satisfied. This is because we can set all other network weights to 0 and adjust the bias terms in the last layer to output any value of $\theta \in \mathbb{R}^d$. %model all densities without conditioning on $X$. \sj{to elaborate this more}

Shannon mutual information is a measure of changes in entropy when conditioning on new variables:
% \js{the two $\Omega$ are not the same for entropy and conditional entropy, why not use the $\Omega$ for conditional entropy always? in entropy your input is $\varnothing$ anyways, the only fix you need is $\gX \cup \{\varnothing\}$ for the domain of $f$}:
\begin{align}
\label{eq:mutinf}
I(X; Y) = H(Y) - H(Y | X) = H_{\Omega^\n}(Y) - H_\Omega(Y | X)
\end{align}

Here, we will use predictive $\F$-entropy to define an analogous quantity, $I_{\F}(X \rightarrow Y)$, to represent the $\text{\it{change}}$ in predictability of an output variable $Y$ when conditioned on $X$. %We use the predictive $\F$-entropy to define the predictive $\F$-information:

\begin{definition}[Predictive $\F$-information]
\label{def:f-information}
Let $X,Y$ be two random variables taking values in $\mathcal{X}, \mathcal{Y}$. Let $\mathcal{P}(\mathcal{Y})$ be the set of all discrete probability distributions over $\mathcal{Y}$. Let $\Omega=\{f:\mathcal{X} \rightarrow \mathcal{P}(\mathcal{Y})\}$, $\mathcal{F} \subseteq \Omega$ and $\F^\n = \{f: \{\n\}\rightarrow g(x)| \forall x \in \mathcal{X}, \forall g \in \F\}$. Assume $\F$ is optional-ignorance w.r.t $\F^\n$, then the predictive $\F$-information from $X$ to $Y$ is defined as
\begin{equation}
I_\F(X \rightarrow Y) = H_{\F^\n}(Y) - H_\F(Y | X)
\end{equation}
\end{definition}

The definition of $\F^{\n}$ ensures that conditioning on $X$ cannot increase the predictability of $Y$ simply by virtue of a more expressive model, without needing any information from $X$. We show in Proposition \ref{prop:subcase} and Appendix \ref{mini} that the optional-ignorance guarantees the non-negativity of $\F$-information.

\subsection{Alternative Attempt at Definitions and Notations}
